When Not to Trust Language Models: Investigating Effectiveness of Parametric and Non-Parametric Memories

Despite their impressive performance on diverse tasks, large language models (LMs) still struggle with tasks requiring rich world knowledge, implying the limitations of relying solely on their parameters to encode a wealth of world knowledge. This paper aims to understand LMs' strengths and limitations in memorizing factual knowledge, by conducting large-scale knowledge probing experiments of 10 models and 4 augmentation methods on PopQA, our new open-domain QA dataset with 14k questions. We find that LMs struggle with less popular factual knowledge, and that scaling fails to appreciably improve memorization of factual knowledge in the long tail. We then show that retrieval-augmented LMs largely outperform orders of magnitude larger LMs, while unassisted LMs remain competitive in questions about high-popularity entities. Based on those findings, we devise a simple, yet effective, method for powerful and efficient retrieval-augmented LMs, which retrieves non-parametric memories only when necessary. Experimental results show that this significantly improves models' performance while reducing the inference costs.

==> sections/intro_prev.tex <==
\section{Introduction}
Large language models (LMs; ~\citealt{brown2020language,chowdhery2022palm}) have shown to be competitive on diverse NLP tasks, include knowledge-intensive tasks that require fine-grained memorization of factual knowledge~\cite{petroni-etal-2021-kilt}. 
Recent work also shows that by prompting LMs, one can even retrieve their knowledge memorized in their parameters (\emph{parametric-knowledge}) as evidence to be directly used for down-stream question answering (QA) tasks~\cite{yu2022generate}. 
However, LMs also show their limited memorization for less frequent entities~\cite{Razeghi2022ImpactOP,llm_longtail}, and they are prone to hallucinations~\cite{shuster2021retrieval} or generate biased outputs~\cite{schramowski2022large}.
Incorporating \emph{non-parametric knowledge} (i.e., retrieved text chunks) largely help LMs to overcome those issues~\cite{llm_longtail}, it is still unclear when parametric knowledge only suffers and how non-parametric memories help.  
% \daniel{since the next paragraph is discussing "parametric" knowledge, we probably should define it and contrast it with "retrieved" knowledge.}

\begin{figure}[t!]
\includegraphics[width=8cm]{figures/teaser_pop.png}\caption{
Relationship between popularity and model performance. \akari{add nice and clear teaser figure as in Colin's paper}
} \label{fig:teaser}
\end{figure}

This work provides a systematic evaluation schema to answer when we {\it should not} rely on the LMs' parametric knowledge and what factors affect their memorization behaviors. 
In particular, we aim to understand the following research questions: 
\begin{itemize}
    \item RQ1: how much factual knowledge is memorized by LMs and what factors affect the memorization? (Section~\ref{sec:analysis_parametric})
    \item RQ2: can non-parametric memories help the shortage of parametric memories of LMs? (Section~\ref{sec:analysis_non_parametric})
    \item RQ3: can we build a system to adaptively combine non-parametric and parametric memories? (Section~\ref{sec:adaptive_retrieval})
\end{itemize}

We first construct X, a large-scale entity-centric QA datasets using WikiData, across diverse relationship types and entity popularity---how often people visit their Wikipedia pages to learn about it. Unlike existing benchmarks that are often biased towards popular entities and exhibit leakage between training and test splits~\cite{lewis2020question}, our queries are sampled uniformly \alex{they actually aren't sampled uniformly from WikiData. We are more likely to sample entities that are more frequent in C4} from the popularity-based distributions, and thus it helps us to test models' true abilities on long-tail distributions. 

We evaluate GPT-2~\cite{radford2019language}, T0~\cite{sanh2021multitask}, OPT~\cite{zhang2022opt}, and GPT-3~\cite{brown2020language} on our benchmark without any fine-tuning. 
Experimental results demonstrate that LMs' memorization is often limited to the most popular entities and even 175B GPT-3 fails to answer for the majority of the long-tail distributions, and their memorization varies across different relationship types. In particular, we observe strong positive correlations (number) between GPT-3's accuracy and the subject entities' popularity. 
Furthermore, LMs' worse reliability on less popular entities means that they are more likely to hallucinate, rely on stereotypes, or otherwise fail to be helpful, honest, and harmless for questions about less popular entities.

\raj{We next investigate whether a semiparametric approach that augments the LM with retrieved evidence can help mitigate the low performance on questions about less popular entities. We find that is indeed the case. Specifically, we found that retrieval-augmented LMs are particularly competitive when the subject entities are not popular (xx.x\% improvement). We also, surprisingly, find that retrieval augmentation can hurt the performance on questions containing popular entities as retrieval can add noisy and irrelevant context.}
To mitigate those problematic behaviors, we evaluate the retrieval-augmented LMs, where documents retrieved by an off-the-shelf retrieval system to be fed with the queries to the LMs. 
We found that those prediction errors can be mitigated by leveraging non-parametric knowledge 
Specifically, we found that retrieval-augmented LMs are particularly competitive when the subject entities are not popular, while LMs often outperform their retrieval-augmented counterparts in popular entities \raj{It might be good to give an explanation about why LMs outperform for popular entities. Is it because the retrieval sometimes adds irrelevant documents to the corpus?}.
Moreover, smaller LMs can outperform 10x bigger LMs when it is augmented by non-parametric knowledge.
We found that recent generative retrieval approaches such as \citet{yu2022generate} exhibits biases similar to the LMs without retrieval. \raj{The last sentence feels a little out of place, since we never mentioned about generative retrieval before.} 

Based on the findings, we introduce a simple approach to adaptively combine parametric knowledge and non-parametric knowledge based on how likely the LMs only fail, and demonstrate that this further improves the performance on X. 
We further evaluate this hypothesis on widely-used QA datasets (X, Y, Z) and confirms that it stands on those distastes as well, shedding the light on promising model development direction, where a system learns to decide if they generate its parametric knowledge or leverage its non-parametric knowledge to build an efficient, powerful and reliable systems. 
% Our contributions are as follows:
% \begin{itemize}
%     \item We introduce X, a new large-scale entity-centric QA dataset with fine-grained relationship types and entity popularity covering long-tail distributions (Section~\ref{sec:dataset}).
%     \item We evaluate diverse LMs with varying number of the parameters on X, and show they struggle in less popular entities and relationship types, as well as their problematic behaviors when they don't memorize (Section~\ref{sec:analysis_parametric}).
%     \item We demonstrate retrieval-augmented LMs can mitigate them, and adaptively combining them based on how likely LMs fail gives further improvements on X, as well as real-world QA datasets (Section~\ref{sec:analysis_non_parametric}). 
% \end{itemize}
\raj{General comments on the intro: I think in the current intro, the role of relation types is not captured well. For example, some questions are intrinsically hard to answer even if they belong to a popular entity but even within each relation type, we see a correlation between performance and entity popularity. I think it will be also good to mention how we get the entity popularity briefly in the intro.}

% , indicating that even with better prompting
% , LMs {\it should not} be used as a signle knowledge source,
% Together we suggest the limitations and potential harms of using the LMs’ parametric memories as a single knowledge source, and the effectiveness of combining LMs with non-parametric memories to build reliable NLP systems. 

% Large language models (LMs) have shown to memorize diverse factual knowledge~\cite{brown2020language}. 

% Large language models (LLMs) have shown to memorize diverse factual knowledge~\cite{brown2020language}, 

% \begin{itemize}
%     \item LMs factual knowledge; gen-read or recite ; memorization
%     \item LM failures can be harmful~\cite{parrish-etal-2022-bbq, Askell2021AGL}
%     \item lack of systematic analysis and understand what factors contribute to memorization in the area of factual knowledge
%     \item introduce new benchmark to incorporate relationship types as well as popularity information
%     \item evaluate many diff models and found that ...
%     \item retrieval augmented generations
%     \item future suggestions
% \end{itemize}
